LACE: Controlled Image Prompting and Iterative Refinement with GenAI for Professional Visual Art Creators

We present LACE, a hybrid Human-AI co-creative system integrated into Adobe Photoshop supporting turn-taking and parallel interaction modes for iterative image generation. Through a study with 21 participants across representational, abstract, and design tasks, we found turn-taking preferred in early stages for idea generation, and parallel modes suited for detailed refinement. While this shorter workshop paper provides key insights and highlights, the comprehensive findings and detailed analysis are presented in a longer version available separately on arXiv.

==> Files/2-Related_Work.tex <==
\section{RELATED WORK}
\subsection{Support Creativity with Computational Tools}
In the field of creativity support, researchers have explored questions including identifying challenges, facilitating cognitive processes, and balancing user control with computational assistance. Prior research has found that creative work often requires the integration of a large amount of original assets and iterative refinement~\cite{okada2024process, daniel2022creative, wilson2012facing}, which is highly repetitive and laborious. 

With the rise of AI, models such as ControlNet~\cite{zhang2023adding}, LoRA~\cite{hu2021lora}, in-painting~\cite{lugmayr2022repaint}, or latent space editing techniques~\cite{Kim2021GanImageEditing, Endo2022User‐Controllable} are able to enhance control over style and composition. Furthermore, with generative AI models such as DALL$\cdot$E~\cite{ramesh2021zero, ramesh2022hierarchical} and DeepArt~\cite{wang2023deepart}, creators are able to create content simply with textual or visual inputs. However, stand-alone features cannot satisfy diverse needs from professional creators and their practical needs. Meanwhile, we have seen a growing interest in designing AI-empowered interactive systems~\cite{hutson2023expanding, choigenerative, voleti2022smpl,lu2024flowy,lu2024misty}. Following a user-centered design process, they allow creators to focus on conceptual and artistic aspects. 

Differently, LACE presents a hybrid method of combing state-of-the-art image generation models with professional editing tools to both unleash the power of generative models and improve their usability.


\subsection{Creativity Support for Digital Art Creators}
Generative AI has especially advanced creativity support for visual artists, especially image, user interface, and graphic designers. Techniques such as sketch- or image-based prompting~\cite{feng2024item, yang2024fine}, as well as methods like prompt-to-prompt editing~\cite{prompt2Prompt}, provide fine-grained control over AI-generated content. These tools allow creators to guide AI systems using sketches, images, or textual inputs, aligning outputs with artistic intentions. 

However, prior research has also shown that creators heavily rely on iterative workflows to refine their creations~\cite{bigelow2016iterating, cassab2019three, gulay2019integrated, jacobs2018extending}, which emphasize real-time feedback, seamless transitions between tools, and precise control over details. Iterative processes enable creators to experiment, adapt, and develop ideas progressively rather than following rigid plans~\cite{chan2015importance, tang2024exploring}. Existing tools often fail to fully support these workflows, requiring users to switch between platforms and disrupting creative continuity. \looseness=-1

LACE specifically targets the needs of visual art creators by enabling, and maintaining coherence across iterations. It exemplifies a complete solution that combines both automatic generation from end-to-end models and user direct manipulation.

\subsection{Adapting AI-empowered Tools for Professional Creators}
Integrating AI with professional art workflows requires a human-centered approach that prioritizes usability and minimizes disruption~\cite{freese2023ai}. Studies indicate that artists prefer AI tools that augment rather than replace their creative processes, retaining control and authorship over their work~\cite{lovato2024foregrounding, shi2023understanding}. While some AI-assisted tools offer advanced features, their lack of compatibility with professional-grade software limits their adoption \cite{pan2024textit, russo2024navigating}. More recently, systems such as MIMOSA~\cite{ning2024mimosa} and PodReels~\cite{wang2024podreels} have exemplified the effectiveness of AI extensions in professional video editing tools such as Premiere Pro for video creators. Additionally, studies have shown that real-time feedback enhances creators' satisfaction and sense of ownership \cite{long2024not, rafner2023creativity, sun2024generative}. 

The design of LACE was inspired from previous work of integrating AI automation into creators' established workflows. In LACE, users are able to manage AI-generated elements as separate layers and to control object-level details, such as hue and saturation, independently. Additionally, LACE introduces an adjustable pipeline that allows creators to fine-tune the balance between manual and AI-assisted edits. 

% \section{RELATED WORK}
%     \subsection{Creative Workflows for Professional Artists}
%         Professional artists possess advanced expertise and require precise control over their creative processes \cite{okada2024process, daniel2022creative, wilson2012facing, eindhoven1952creative, ecker1963artistic}. They rely on tools that support control, customization, and continuous iteration across various fields including images, paintings, photography, and videos \cite{qiu2023application, montabone2010beginning, upadhyeai}. It is crucial for the workflows to support these artists to capture real-life moments in photography, exercise creative freedom in painting, and blend various elements to make careful adjustments in digital images \cite{yan2016automatic, aparna2017swarm, barni2018cnn}. 
%         Artists engage in fluid, iterative workflows, evolving their ideas in real-time rather than following a predetermined plan \cite{bigelow2016iterating, cassab2019three, gulay2019integrated, jacobs2018extending}. This iterative nature allows for spontaneous creativity and adaptability. However, the necessity to switch between multiple tools can disrupt workflow continuity and hinder the coherence of iterative refinements, making it challenging to maintain a seamless creative journey\cite{Visual_thinker}. There are also works that starts to investiaget how to make up the lost support for a specific step in content creation by building extensions on exisitng tools to streamline the workflow content creators, e.g. MIMOSA~\cite{mimosa} mititagating the gap of editing audio effects for video editing, Podreels~\cite{podreels}, extends the power of trasiotnal profesional tools i.e. premiere pro by leveraging its infrustrurue to make variation on the source video fiel and hlep the users make a teaser video out of a very long video. 
        
%         With the development of artificial intelligence, intelligent workflows with AI embedded offer the potential to automate repetitive tasks such as rendering\cite{marelli2022designing, bussell2023generative, heikkinen2022digital} and image editing \cite{hutson2023expanding, anantrasirichai2022artificial, choigenerative, voleti2022smpl}, enabling artists to focus on more creative aspects. For example, tools like Adobe Sensei incorporate human-AI collaboration pipelines that offload routine tasks while preserving creative control. Additionally, AI-based creation tools such as DALL$\cdot$E \cite{ramesh2021zero, ramesh2022hierarchical} and DeepArt \cite{wang2023deepart} assist in generating and refining content effectively, enhancing the creative process by simply integrating these models with existing workflows. 
        
%      \subsection{AI-Assisted Technology for Creativity}
%         Generative AI models like diffusion models \cite{StableDiffusion} and image transformers \cite{image_transformer} have made art creation more accessible by generating high-quality images from textual descriptions \cite{StackGAN, creativity_text2img}. While beneficial for a broader audience, these models pose challenges for professional artists who require precise and nuanced control. For example, text prompts can be vague and fail to capture specific artistic intentions, leading to outputs that need substantial refinement \cite{wang2023reprompt, wang2024promptcharm}. There are also ewxamples of using ai to facilitate the UI design such as MISTY~\cite{misty} and flowy~\cite{flowy}

%         Researchers have addressed these limitations by exploring alternative input modalities. Image-guided or drawing-guided AI systems \cite{semantic_segmentation_diffusion,cao2023animediffusion, lugmayr2022repaint} and multimodal inputs combining text and images \cite{Multimodal_guided_diffusion} allow artists to provide more direct and detailed guidance during image generation from cross-modality. These approaches enhance intuitiveness and usability, facilitating a seamless integration of artistic intent with machine-generated content.
        
   
%     \subsection{Enhancing Control in AI Image Generation}
%         To provide artists with finer control, techniques such as image-based prompting enable the use of sketches or existing images to guide AI generation \cite{feng2024item, yang2024fine}. Methods like ControlNet \cite{zhang2023adding} and prompt-to-prompt editing \cite{prompt2Prompt} introduce mechanisms to adjust latent space parameters or manipulate specific features post-generation. However, these tools often operate outside professional editing environments and may not align with the iterative workflows of professional artists.

%         To solve such a research gap, our work builds on these efforts by integrating image prompting within professional tools like Photoshop. By allowing artists to use familiar features—such as blending modes and layer adjustments—we enable fine-grained control over AI-generated outputs within their established workflows.
        
        
%     \subsection{Integrating AI with Established Workflows}
%         Integrating AI with professional art workflows requires a human-centered approach that prioritizes usability and minimizes disruption \cite{freese2023ai}. Studies indicate that artists prefer AI tools that augment rather than replace their creative processes, retaining control and authorship over their work \cite{lovato2024foregrounding, shi2023understanding}. While some AI-assisted tools offer advanced features, their lack of compatibility with professional-grade software limits their adoption \cite{pan2024textit, russo2024navigating}.

%         Our system addresses this gap by embedding AI capabilities directly into professional tools. By integrating AI into environments like Photoshop, we ensure that artists can seamlessly incorporate AI-generated content without altering their established workflows, maintaining coherence and control in iterative creative tasks.

        
%     \subsection{Supporting Iterative Creative Processes}
%         Iteration is fundamental to the creative process, allowing artists to refine and enhance their work through repeated cycles of feedback and adjustment. For example, Chan \textit{et al.} \cite{chan2015importance} highlights how iteration contributes significantly to creative conceptual combinations, underscoring its importance in artistic endeavors. Existing AI tools that generate images from scratch each time can disrupt visual coherence and hinder the progressive development of ideas. Tang \textit{et al.} \cite{tang2024exploring} discusses the impact of AI-generated image tools on users in the art design field. While interactive generative tools facilitate dynamic modifications, they often require artists to switch between platforms, causing workflow interruptions.

%         Our system introduces a dual-feedback-loop mechanism within professional-grade tools, enabling artists to balance AI-generated input with manual adjustments iteratively. This approach maintains coherence and continuity across iterations, aligning with artists' natural workflows and enhancing the creative experience.
        
%         Empirical studies show that iterative workflows enhance artists' sense of ownership and satisfaction \cite{long2024not, rafner2023creativity, sun2024generative}. By providing real-time feedback and enabling incremental improvements, AI-assisted tools that support iteration foster a more engaging and fulfilling creative journey.
        
                
   

==> Files/5-Result.tex <==
\section{Preliminary Study and Findings}
\label{sec:prelim-study}

We conducted a user study with 21 participants (ages 20--27, varying Photoshop experience) to compare LACE (\textbf{W3}) against two baseline workflows: text-to-image generation (\textbf{W1}) and text-to-image with a reference image (\textbf{W2}). Participants completed one of three art tasks: representational, abstract, or a pixel-art design challenge. We measured satisfaction, ownership, usability, and artistic perception on 7-point Likert scales.

\vspace{0.5em}
\noindent\textbf{Key Findings.}
\begin{itemize}[leftmargin=*]
    \item \textbf{LACE Enhances User Experience.} Participants rated LACE significantly higher than W1 and W2 on usability, ownership, and satisfaction, with 71.4\% selecting LACE as their preferred workflow.
    \item \textbf{Increased Control \& Reduced Randomness.} Unlike text-based prompting, LACE allowed precise adjustments through Photoshop’s layer-based editing, making iteration more predictable and intuitive.
    \item \textbf{Deeper Engagement.} Participants spent more time refining their work in LACE, particularly in structured design tasks, suggesting greater creative investment.
\end{itemize}

Overall, LACE provides stronger user control and creative coherence than text-only approaches, improving professional usability while integrating AI-assisted workflows into industry-standard tools. Future work will refine its interface for more complex design tasks.

==> Files/7-Limitations_and_Future_Work.tex <==
% \section{LIMITATIONS}

% \textbf{Participant Background and Expertise}: 
% The insights from our participants may not apply to all future users of systems like LACE, as the study primarily involved individuals with backgrounds in digital art or computer science. Participants’ varying levels of experience with AI tools and Photoshop likely contributed to differences in completing creative tasks. For instance, in Workflow 2 (W2 in table~\ref{tab:testing_material}), participants struggled with leveraging latent coherence in art iterations due to unfamiliarity with advanced AI concepts and the ComfyUI interface. Similarly, in Task 2 (T2 in table~\ref{tab:testing_material}), participants without a traditional art background had difficulty creating prompts for abstract art because of limited experience in conceptualizing such work. The 30-minute time constraint for each task may have exacerbated these differences, introducing bias into the results.

% \textbf{Study Design Constraints and Generalizability}: 
% The study’s design limitations may have influenced results and generalizability. The 30-minute task duration restricted participants’ deep engagement, potentially affecting performance and satisfaction. Art creation is time-consuming and iterative, requiring extended reflection and revision. The short duration may not accurately capture participants’ true experiences, as mental states like stress, fatigue, or frustration could have influenced responses. The novelty of the LACE system led to initial positive reactions, but these may not reflect long-term perceptions. Participants might have been enthusiastic due to the system’s novelty, which could wane over time. Future studies should allow more extended interaction periods to assess sustained user engagement, satisfaction, and the tool’s effectiveness in supporting diverse creative processes.

% \textbf{Survey Design and Bias}: 
% Many survey questions framed artistic aspects like satisfaction, ownership, and `Art' assumption of participants’ understanding or interest in artistic creation. This may not hold for all users. Non-artists might be influenced by unfamiliar terminology or processes, leading to biased responses. They might interpret questions differently or struggle to evaluate outputs based on artistic standards, skewing assessments across disciplines. Future studies should adjust language and focus to accommodate diverse backgrounds for more accurate results.

==> Files/8-Conclusion.tex <==
\section{Conclusion}
    We presented LACE, an image-prompting system designed to enhance professional artists’ workflows by integrating AI-driven content generation into established creative environments. Through a user study involving 21 participants, we demonstrated the usability of LACE in providing fine-grained control over image prompts and enables coherent iterative refinement. Participants reported a stronger sense of ownership, and viewing their output as more artistic when using LACE.
